Cocktail HuBERT: Generalized Self-Supervised Pre-training for Mixture and Single-Source Speech

Self-supervised learning leverages unlabeled data effectively, improving label efficiency and generalization to domains without labeled data. While recent work has studied generalization to more acoustic/linguistic domains, languages, and modalities, these investigations are limited to single-source speech with one primary speaker in the recording. This paper presents Cocktail HuBERT, a self-supervised learning framework that generalizes to mixture speech using a masked pseudo source separation objective. This objective encourages the model to identify the number of sources, separate and understand the context, and infer the content of masked regions represented as discovered units. Cocktail HuBERT outperforms state-of-the-art results with 69% lower WER on multi-speaker ASR, 31% lower DER on diarization, and is competitive on single- and multi-speaker tasks from SUPERB.

==> tables/algorithm.tex <==
%\begin{minipage}[t!]{\textwidth}
%\begin{singlespace*}
\begin{table*}[t]
\hline
\vspace{2pt}
\textbf{Algorithm 1}: Overlapped Speech Simulation
\vspace{2pt}
\hline
\small
$ $ 1: given a batch of speech utterances $U = {u^i}^{B}_{i=1}$ with batch size $B$, mixing probability $p$, a set of DNS noises \cite{Reddy2021} $N = {n^i}^{M}_{i=1}$, with size $M$,   

\hspace{10pt} mixing noise probability $p_n$, max-num-speakers $ms$, the min/max location to mix relative to primary start $O_{min}$, $O_{max}$, the min/max 

\hspace{10pt} length ratio of primary length $L_{min}$, $L_{max}$ for determining mix length

$ $ 2: choose $S$ utterances $U^S \subset U$ by Bernoulli sampling with probability $p$ 

$ $ 3: choose $n$ number of speakers to mix from discrete uniform distribution with probability $P(n = x)=\frac{1}{ms - 1}, x \in \{2, ..., ms\}$

$ $ 4: \textbf{for} each primary utterance ${\textnormal u}^{pri} \in U^S$ \textbf{do}

$ $ 5: \hspace{5pt} calculate the energy of the primary utterance $E^{pri} \xleftarrow{} \frac{\sum{{\textnormal u}^{pri} . {\textnormal u}^{pri}}}{len({\textnormal u}^{pri})}$

$ $ 6: \hspace{5pt} let $X$ be the list of utterances to mix with

$ $ 7: \hspace{5pt} \textbf{for} $n$ number of speakers \textbf{do}

$ $ 8: \hspace{15pt} sample a random value $v$ from the continuous uniform distribution ${\cal U}(0, 1)$

$ $ 9: \hspace{15pt} \textbf{if} $v > p_n$ \textbf{then} sample an utterance ${\textnormal u}^{sec}$ from discrete uniform distribution with probability $P({\textnormal u}^{sec} = x) = \frac{1}{B}, x \in U, x \notin X$

$ $ 10: \hspace{10pt} \textbf{else} sample a noise ${\textnormal u}^{sec}$ from discrete uniform distribution with probability $P({\textnormal u}^{sec} = x) = \frac{1}{M}, x \in N$

%$ $ 13: \hspace{6pt} \textbf{end if}

$ $ 11: \hspace{10pt} add ${\textnormal u}^{sec}$ to $X$

$ $ 12: \hspace{10pt} sample the mixing energy ratio $r$ from the continuous uniform distribution ${\cal U}(-5, 5)$

$ $ 13: \hspace{10pt} sample the mix length $l$ from discrete uniform ... \maryam{update}

$ $ 14: \hspace{10pt} sample a start position $s^{pri}$ from discrete uniform ... \maryam{update}

$ $ 15: \hspace{10pt} calculate the energy of the secondary utterance $E^{sec} \xleftarrow{} \frac{\sum{{\textnormal u}^{sec} . {\textnormal u}^{sec}}}{len({\textnormal u}^{sec})}$

$ $ 16: \hspace{10pt} calculate the mixing scale $scl \xleftarrow{} \sqrt{\frac{E^{pri}}{10^{\frac{r}{10}}E^{sec}}}$

$ $ 17: \hspace{10pt} ${\textnormal u}^{pri}[s^{pri}: s^{pri} + l] \xleftarrow{} {\textnormal u}^{pri}[s^{pri}: s^{pri} + l] + scl \times {\textnormal u}^{sec}[0 : l]$

%$ $ 19: \hspace{2pt} \textbf{end for}

%$ $ 20: \textbf{end for}

$ $ 18: \textbf{return $U$}
\vspace{2pt}
\hline
\end{table*}
%\end{singlespace*}
%\end{minipage}
